Interpreting the Robustness of Neural NLP Models to Textual Perturbations

Modern Natural Language Processing (NLP) models are known to be sensitive to input perturbations and their performance can decrease when applied to real-world, noisy data. However, it is still unclear why models are less robust to some perturbations than others. In this work, we test the hypothesis that the extent to which a model is affected by an unseen textual perturbation (robustness) can be explained by the learnability of the perturbation (defined as how well the model learns to identify the perturbation with a small amount of evidence). We further give a causal justification for the learnability metric. We conduct extensive experiments with four prominent NLP models -- TextRNN, BERT, RoBERTa and XLNet -- over eight types of textual perturbations on three datasets. We show that a model which is better at identifying a perturbation (higher learnability) becomes worse at ignoring such a perturbation at test time (lower robustness), providing empirical support for our hypothesis.

==> comments.tex <==
Response to SACs:

Dear SACs,

Thank you for taking the time to review our paper. We appreciate the reviewers' thoughtful feedback. We are glad to see that reviewers have identified the following strengths of our work:
- clear and interesting research questions (NKmd, 7eV4)
- novel design of the learnability metric (VXhG, V5kc)
- extensive experiments with convincing results (NKmd, 7eV4)
- the potential for guiding future works on improving model robustness (VXhG, V5kc)

However, we would like to draw your attention to reviewer 7eV4's confidence score of 1 and admission that this paper is not within their area of expertise. We would also like to clarify some misunderstandings:

*Re: Random perturbation does not guarantee a perfect decoupling of confounders from the causal graph (7eV4).*

We do not agree with the reviewer's argument. If the perturbation (P) causes changes on latent features (i.e., P -> T -> L in Figure 2), then T should be called a mediator instead of a confounder. So randomization can still remove confounders in the causal graph.

*Re: Eq2 seems to have an assumption that the test accuracy of the original test set is invariant against training with augmentation or not (VXhG).*

In this work, we focus on the robust accuracy (Section 2.1), which is accuracy on the perturbed test set. We do not assume that the test accuracy of the original test set, a.k.a in-distribution accuracy, is invariant. We hypothesize that training with augmentation might incur a drop in in-distribution accuracy, which is not explored in this work. It would be interesting to investigate the trade-off between robust accuracy and in-distribution accuracy in the future.

*Re: It would be great to have a paragraph on the limitations of your study/conclusions (kdPi).*

We have already discussed some limitations in Section 5, which we will expand in the camera-ready. For example, some perturbations may deviate from the conclusion if they are symmetric or label-inconsistent or already exist in the original data  (we have these assumptions for perturbations in Section 4.1). We also plan to experiment with more architectures, including Logistic Regression, Support Vector Machines, Naive Bayes.

*Re: Some perturbations in Figure 3 have altered the results (labels) of the original instances/pairs (V5kc).*

The last two perturbations in Figure 3 look more damaging than others but they are still readable for humans. Since they are visual perturbations (e.g., e -> 3), the labels do not change after perturbations. The results for these perturbations have already been included in the numbers in Table 3 and dots in Figure 5-7 and conform to our conclusions. Furthermore, we could do some analysis on a subgroup of perturbations.

Finally, we agree with the meta-reviewer that we should clarify the definitions and assumptions, expand the analysis of the experiments and discuss the limitations of our study/conclusions. We will revise our paper accordingly in the camera-ready.


*****************************************************************

I. Meta-review
1. There are some questions/discussions on clarifying the definitions and assumptions which should be improved (VXhG)

> Yunxiang: Addressed.

2. Reviewer NKmd and V5kc have some suggestions for expanding the discussions of the experiments, related works, and figure captions, which all seem reasonable.

> Yunxiang:

3. Hinted in the comments of 7eV4, it would be great to have a paragraph on the limitations of your study/conclusions (what form of perturbations/architectures might deviate from this conclusion?)

> Yunxiang: already discussed some limitations in Section 5. could expand it. Deviation situations: perturbations that are symmetric or label-inconsistent or already exist in the original data  (Section 4.1); architectures: need more experiments. LR SVM NB
Most important features learned by an SVM classifier trained on TF-IDF bag of words. following Kaushik et al., 2020

*****************************************************************

II. Reviewer VXhG
1. Eq2 seems to have an assumption that the test accuracy of the original test set (D_test) is invariant against training with augmentation or not. This might not be true in practice. So the delta score only shows F1 difference on the perturbed set. If the perturbed set has no example overlap with the original D_test, then what are the delta scores for original testing F1s? Is there something interesting to see?

> Yunxiang: Addressed. (Sec. 5)

we focus on robust accuracy. indistribution
accuracy is beyond the scope.
Tu et al., 2020: There is a trade-off between in-distribution
accuracy on the independent and identically distributed
(i.i.d.) test set and robust accuracy on
the challenging dataset. Nevertheless, recent empirical
results have suggested that self-supervised
pre-training improves robust accuracy, while not
using any task-specific knowledge nor incurring indistribution
accuracy drop

2. What is the separation between accuracy and robustness. Would like to see a discussion/treatment on this.

3. Several of the perturbation methods are effectively replacing tokens with [UNK] in transformer models. This is a limitation of textual perturbation that it wipes out the features this paper wants to perturb. Also, does it have something to do with the high variance on the low learnable end in Fig 1?

4. Spearman correlation 0.6 is not a strong number (but said to be "strong" in Sec 4.4). In Tab 3, it seems the correlation is a data-by-data thing, e.g. Yelp is strong but the other two data are moderate.

> Yunxiang: Ignored.

0.6 is strong according to https://www.statstutor.ac.uk/resources/uploaded/spearmans.pdf 
reveals signals in dataset / perturbation feature already exists in datasets. 

*****************************************************************

III. Reviewer NKmd
1. There is a limited discussion of the results. The main results appear on the second-to-last page and there is not much room dedicated to answering follow-up questions about the results. The authors could devote more space to discussing the relationship and its implications; having established a causal connection between learnability and robustness, they could delve deeper into what types of perturbations represent outliers. Similarly, the discussion of the results on augmentation are minimal, with most of the paper dedicated to the learnability vs robustness result.

2. I personally would like to see more discussion on the interaction between BPE and learnability/robustness. The following paper is a good reference for the interaction between BPE and robustness: https://arxiv.org/abs/2104.08211.

3. Relatedly, the related works section is quite sparse. There is a unexplored connection between the work here and work on robustness to spurious correlations (e.g. https://arxiv.org/abs/2005.04345).

4. I find Fig. 1 almost impossible to read; it only clearly shows the relationship between post augmentation delta and robustness, when the core contribution of the paper is the relationship between the learnability and robustness. In the appendix, Figs. 5-7 (a and b) are much clearer, and I would advocate for Fig 1 being replaced with something like Fig 5 (a,b).

> Yunxiang: Agreed. will revise accordingly.

*****************************************************************

IV. Reviewer 7eV4
1. Although perturbation is purely random, it does not guarantee a perfect decoupling of confounders from the causal graph. It could happen that when you perturb a sentence, the perturbation also causes changes on confounder features, i.e., P' -> P' will cause T -> T' -> L'.

> Yunxiang: Since the edge goes from P to T, T is called a mediator instead of a confounder. 

2. The key finding of this paper is the negative correlation between learnability and robustness, this also leads to major claims made by the author. However, the only experimental evidence to support these findings is Table 3. Further evaluation would help substantiate the claims, e.g., some human evaluation.

3. Would be helpful to provide a running example to help understand learnability.

> Yunxiang: case study or visualization is helpful though difficult to design. 

*****************************************************************

V. Reviewer V5kc
1.Some perturbations in Figure 3 have altered the results (labels) of the original instances/pairs, e.g., the last two perturbations have damaged the semantics of the original input. Are the results on these data persuasive? 

> Yunxiang: mapping rules between perturbed and original data.

2. This work lacks detailed analysis on the results of Table 2 (see comments). 

3. This work lacks the analysis of the impact of augmented data size.

> Yunxiang: future work

4. 423~426: Is the "effects on the tokenization process" main reason?

> Yunxiang: Addressed.

educated guess

5. 427~434: "white_space_perturbation" also affects the tokenization, as the white space is randomly inserted into a word.

> Yunxiang: Addressed.

different patterns of destroying tokenization.

6. In table 2, why TextRNN is more sensitive to "insert abbreviation" than "shuffle word"?

7. What does Table 3 talk about?

> Yunxiang: core results supporting hypothesis 1 and 2.

8. I think Parts a and b in Figure 5-7 are more important, and should be shown in the paper text.

> Yunxiang: Addressed.

Agreed. TODO

9. Some perturbations in Figure 3 have altered the results (labels) of the original instances/pairs, e.g., the last two perturbations and the "shuffle word", what is the performance of augmentation based on these perturbations?

> Yunxiang: included in the results of Table 3. could do some separate analysis.
